On Performance Debugging of Unnecessary Lock Contentions on Multicore Processors: A Replay-based Approach

Locks have been widely used as an effective synchronization mechanism among processes and threads. However, we observe that a large number of false inter-thread dependencies (i.e., unnecessary lock contentions) exist during the program execution on multicore processors, thereby incurring significant performance overhead. This paper presents a performance debugging framework, PERFPLAY, to facilitate a comprehensive and in-depth understanding of the performance impact of unnecessary lock contentions. The core technique of our debugging framework is trace replay. Specifically, PERFPLAY records the program execution trace, on the basis of which the unnecessary lock contentions can be identified through trace analysis. We then propose a novel technique of trace transformation to transform these identified unnecessary lock contentions in the original trace into the correct pattern as a new trace free of unnecessary lock contentions. Through replaying both traces, PERFPLAY can quantify the performance impact of unnecessary lock contentions. To demonstrate the effectiveness of our debugging framework, we study five real-world programs and PARSEC benchmarks. Our experimental results demonstrate the significant performance overhead of unnecessary lock contentions, and the effectiveness of PERFPLAY in identifying the performance critical unnecessary lock contentions in real applications.

==> discussion.tex <==
The overall goal of \textsc{PerfPlay} is to identify the beneficial code regions and help developers understand ULCP problems. However, there are still some promising problems needed to be paid attention to and discussed.
\begin{comment}
\textbf{Optimization Reliability:}
%Generally, different inputs will produce different outputs for the multi-threaded applications.
%At the beginning of the design choice, we once thought about static exploration, which is able to expand all potential paths of programs for the analysis. But we later abandon this idea for the redundant ULCP-irrelevant path information it produces and the lose of such detailed information as pointer accesses, which is the crux to the identification of ULCPs. Therefore,
\textsc{PerfPlay} adopts a dynamic binary instrumentation method to figure out the beneficial ULCPs based on the specific execution trace, which are inapplicable to guide ULCP performance impact for other execution traces. Even so, it does not hurt the significance of our work since the reported ULCPs are surely identified to have an impact on performance for this specific execution.
%Therefore, the concern, "\emph{are the sets of optimized outputs \textsc{PerfPlay} performs reliable?}", seems to be very practical.
To export the complete ULCP results for each application, we can leverage \textsc{PerfPlay} to repeatedly test the programs with different input sets which can be automatically generated by the state-of-the-art generators \cite{PEX} for high code coverage.
\end{comment}
% Enlightened by the observation from our study that ISOs normally manifest themselves in a specific thread interleaving, we come to the realization that a dynamic approach, using K-constraint to tradeoff the influence of different input, may be a better choice. However, it should be mentioned that the factors $\theta$ and $\overline{\eta}$ are the two empirical values, which depend on the number of input sets as large as possible.
%For these reasons and more, we leveraged the dynamic instrumentation method as our research strategy, which provides an effective and efficient way to tackle the ISO performance bugs. And we argue that the ISO performance bug sets \textsc{PerfPlay} produces are reasonable and reliable.
\begin{figure}[tbp] %Figure 1
\centering
\setlength{\abovecaptionskip}{10pt}
\setlength{\belowcaptionskip}{-10pt}
\includegraphics[scale=0.65]{fig/irrelevant_parts.eps}
\caption{Fine-grained ULCPs within the critical sections. The combinations in the dashed box show the ULCP problem.}
\label{fig:irrelevant_parts}
\end{figure}

\textbf{External ULCP Events:}
All tested applications in our experiments are self-contained. That is, the thread interleaving is affected by internal events, such as thread scheduling, memory reordering, and time variations. \textsc{PerfPlay} performs very well for this type of applications. However, for those applications involving external events (e.g., user input and the arrival of network packets), if the code regions with ULCP problem involve external events, \textsc{PerfPlay} will treat the responsive time caused by external events as a part of performance metrics of such an ULCP. In other words, it increases the proportion $P$ of such an ULCP, and reduces the significance of other real ULCP problems. To tackle this issue, we will ascertain external ULCP events in future work.

\textbf{Fine-grained Optimization of ULCPs:}
%This paper presents three categories of ISOs, on the basis of which appropriate techniques to tackle them are proposed. In addition,
The definition of ULCP in this paper constrains that the \emph{entire} region in two critical sections must be parallelizable. However, the cases of critical sections simultaneously containing the conflicting regions and parallelizable regions are more common in real world. At this point, the unified protection using the same lock for the critical sections produces more fine-grained ULCPs. Figure~\ref{fig:irrelevant_parts}(a) depicts an example of this scenario where two threads concurrently use the same shared data \texttt{C} for the transition assignment. The detailed decomposition of this code, two fine-grained ULCPs of $\sf \langle read(A),read(B)\rangle$ and $\sf \langle write(D),write(E)\rangle$ as shown in Figure~\ref{fig:irrelevant_parts}(b), in fact, can be executed in parallel. To evaluate this problem, one of the most intuitive approaches is to extract fine-grained ULCPs outside the critical sections (as shown in Figure~\ref{fig:irrelevant_parts}(c)). However, this strategy could lead to atomicity violation which produces inconsistent and incorrect results, or some fresh data races conflicting with other shared memory access events. For the integrity of our work, we will focus on the exploration of this topic in future work.

\begin{comment}
\noindent\textbf{Fixing the ISO-performance Bugs in Source Level}.
In this paper, \textsc{PerfPlay} is proposed to provide a series of optimization opportunities for the ISO-performance bugs, mainly including the setting position, optimization proportion and ISO-awareness execution scenarios. All the work is based on program binary level. Another concern, "\emph{How to fix the ISO-performance problems in source code level?}", seems to be more exhilarating.
The contact between source level and binary level is that binary level optimization is one of the many source level optimizations. However, in most cases, the optimization of source level is hard to achieve the same effect as binary level. This is why the optimization opportunities \textsc{PerfPlay} provides is an optimal performance criteria. To fix the ISO-performance bugs in source level, however, there are still many challenges needed to overcome.
1) \emph{Code Readability}. Some safeguard measures for fixing ISO-performance bugs, such as local synchronization and isolation techniques, generally result in very poor code readability. As shown in Figure~\ref{fig:null_lock}, double checking method is very confusing when proposed to optimize synchronization overhead.
2) \emph{Code Reorganization}. Sometimes, a little change of codes, like double checks, is very seldom. In most cases, developers have to reorganize the codes to eliminate ISOs.
3) \emph{Other Concurrent Bugs}. For each type of ISO, one common fixing strategy is to use different lock for different shared data. However, our study proves that this strategy might lead to other concurrent bugs, such as atomicity violation and data races, in source level.
\end{comment}

%To ascertain this issue, we will conduct a study on the exploration of this topic in future work. %Ultimately we call on the developers to try the best to avoid the cases of ISO-performance.%, and we are firmly convinced that each ISO-performance problem can be optimized by a non-ISO approach.


==> study.tex <==
We study the ISO problem on several open-source programs in terms of behaviors, categories, and root causes. %Specifically, a set of micro-benchmarks, with an integrated inclusion of each category as discussed in Section~\ref{sec:category}, is implemented to evaluate the optimizable value of these bugs, and \textsc{PerfPlay}, an ISO-based detector, is proposed to understand the presence and optimization of these bugs in some real-world applications. Table~\ref{table:microbenchmark} shows the concrete composition of micro-benchmark.
\begin{comment}
It is revealed in our study that ISO-problem bugs are involved in every application studied with various forms of manifestation. This section, in the purpose of throwing fresh light on ISO-problem bugs, mainly deals with the issues as following:
\begin{itemize}
  \item What forms do the ISO-problem bugs usually take? Study concerning this issue will facilitate the exposure of different forms of ISO-problem bugs when the software is in service.
  \item What are the root causes of ISO-problem bugs? Study concerning this issue will provide more profound understanding for ISO-problem bugs.
  \item Is there any method to solve ISO-problem bugs of each category based on the understanding of these classified bugs? Study concerning this issue entails an introduction to the relevant previous work so as to tackle the various challenges encountered by ISO-problem bug detection in a more efficient manner.
\end{itemize}
\end{comment}
\subsection{Classification of ISOs}
\label{sec:category}
In this study, ISOs are mainly manifested in the form of lock operation and are classified into three categories according to the shared variable information in the critical sections. To be precise, lock primitive is generally used for the exclusive access to the shared memory locations with a guarantee of the correctness of the program. However, improper use of lock (see section~\ref{study:root_causes}), will lead to a significant performance degradation of a program, which can be reflected in at least three aspects:

(1) \emph{{Null-Lock}} refers to the synchronization pair where there exists no shared-memory access in the critical sections. ISO-problems of this type are usually relatively easy to understand and identify, and they are normally fixed by eliminating the lock operation. The occurrence of null-locks generally comes down to \emph{if-access} and \emph{compiler optimization}. \emph{If-access} allows the shared memory accesses with the prerequisite that the if-condition is true. \emph{Compiler optimization} arises out of the fact that quite a few developers, with bad programming habits, often do some trivial matters in the critical sections.
\begin{figure}[tbp] %Figure 1
\centering
\includegraphics[scale=0.7]{fig/Null_lock.eps}
\caption{An OpenLDAP read-read bug that will waste a great deal of CPU time if a large number of threads call this code simultaneously.}
\label{fig:null_lock}
\end{figure}

(2) \emph{Read-Read} pattern indicates that only shared memory read operations exist between the two critical sections which are mutually exclusive using the same lock. %Figure~\ref{fig:1} illustrates a typical example of \texttt{read-read} synchronization operation.
The performance problem of this type mainly stems from the serial access to the shared memory location, especially for those memory-intensive applications. Performance problems of this type are difficult for compiler or developer to optimize due to the possible overlapping of one synchronization pair of read-read pattern with another relevant write synchronization operation. Usually there are two ways to fix them: i) a conservative optimization using different locks for different shared memory locations as shown in Figure~\ref{fig:1}(b); ii) an aggressive optimization by eliminating the synchronization lock properly. However both ways are likely to encounter the challenge of introducing some data races.

Figure~\ref{fig:null_lock} demonstrates such an ISO-problem bug from OpenLDAP \cite{OpenLDAP}, a lightweight directory access protocol server. This bug causes performance slowdown, that is because it produces a large amount of \textsf{lock/unlock} pairs where no effective execution statement exists if \texttt{dbmfp->ref} is always read by false (line 4). This performance degradation is particularly severe when a large number of threads execute this code at the same time. To optimize the synchronization overhead and corresponding serial overhead, we can use double checks\footnote{Sequential consistency memory model is assumed here.} \cite{double_check}, as shown in Figure~\ref{fig:null_lock}, by first testing the locking criterion without actually acquiring the lock. Only if the locking criterion check indicates that locking is required does the actual locking logic proceed (line 6/9 as indicated in patch).

(3) \emph{Irrelevant Write-Being} pattern occurs in the scenario where more than two memory operations in the critical sections, mutually exclusive using the same lock and located separately in different threads, access their own shared memory location, and at least one of them is the write operation. Similar to read-read pattern, this type of bug is hard to optimize. They are usually fixed by using different locks for different memory locations, however, there are also some special obstacles needed to cope with, such as data races.

%\noindent\textbf{Signal/Wait:}
\begin{comment}
%\noindent\textbf{Barrier:}
\begin{table}[tbp]   %Table
\centering
\small
\caption{Quantity of each category in micro-bechmark}
\begin{tabular}{c|c|c }\Xhline{1pt}
  \textbf{Null-locks}&\textbf{Read-Read}&\textbf{Irrelevant W-being} \\ \hline
  $1\times10^5$&$1\times10^5$&$2\times10^5$ \\ \Xhline{1pt}
\end{tabular}
\label{table:microbenchmark}
\end{table}

\subsection{Data Sets}
Before the study, we need to make a whole evaluation of work significance. Hence, we implement a set of micro-benchmarks with an integrated inclusion of each category as discussed in Section~\ref{sec:category}.

Besides, we select several representative applications from the real-world open sources, including two server systems (OpenLDAP \cite{OpenLDAP} and MySQL \cite{mysql}); three desktop applications (pbzip2 \cite{pbzip2}, transmissionBT \cite{transmissionbt} and handBrake \cite{handbrake}) and all applications from PARSEC benchmark suite \cite{parsec}. %These selections are made as the target of our study for two main reasons.

\begin{enumerate}
  \item They are all widely-used concurrent programs. The reasons for their popularity are various, each enjoying at least one hundred thousand users. Some (e.g., mysql 1994 and OpenLDAP 1998) boast a long history of more than ten years; some (e.g., transmissionBT and handbrake), though lack of adequate maintenance history, are more and more prevalent along with the market demand, attracting us for the emerging program characteristic they reveal; still some others (e.g., PARSEC benchmark) declare to be representative of next generation shared-memory programs for chip multiprocessors as much as possible, thus gaining a foothold in academic.
  \item All of them are open-source concurrent programs which can facilitate our understanding and analysis of the root causes and subsequent effects of ISOs. For example, chances are that we can not confirm the facticity of a latent ISO identified by detectors, and that we wonder about its semantics and detailed context information of execution trace. In such a case, we can refer to the corresponding source locations of ISOs, which can help us develop a more precise and understandable report.
\end{enumerate}
\end{comment}
\subsection{Root Causes of ISOs}
\label{study:root_causes}
There is a large variety of potential root causes for the ISO-performance problems, mainly including coding problem and configuration problem. Among them coding problem is the most common one.
%Our goal in this sub-section is \emph{not} to summarize previously unheard of root causes, but to reconfirm these indeed factors lead to ISO-performance problems. Reasons for the occurrence of ISO we identify are as follows.
\begin{figure}[tbp] %Figure 1
\centering
\includegraphics[scale=0.7]{fig/fastlock.eps}
\caption{A MySQL modular design bug with over synchronization. This bug can be fixed by replacing \texttt{random} with a non-synchronized random number generator.}
\label{fig:fastlock}
\end{figure}
%Specifically, coding problem is a performance problem lying in the inner of the application itself.
%Poorly written application code can result in redundant or unnecessary work.
Here are two reasons of coding problem: 1) Lack of Skills. Programmers, for a lack of abundant personal knowledge, may fail to code each program in a perfect way. %, such as workload mismatch and API misunderstanding.
Meanwhile, they sometimes use many ad-hoc synchronizations (like while-loop, spin-lock) in the multi-threaded applications, 22-67\% of which, unfortunately, may introduce bugs or severe performance issues \cite{Xiong}. Performance problems of this sort are very subtle, and it is generally hard for them to expose themselves in the development of software. 2) Modular Design. In order to shorten the software development life cycle, programmers often adopt the modular design to make sure that everyone has a very clear division of labor and the each final project deliverable provides the interfaces as expected. The most common form of modular idea is using the design of function and macro commands. However, this idea normally brings about some performance loss \cite{Jinguoliang}. For example, Figure~\ref{fig:fastlock} shows a modular design of fast-lock implementation in mysql-5.1. Fast mutex calls \texttt{random}, which is thread safe and uses one mutex in glibc on Linux, to determine the spin wait time. This lock serializes the invocation of \texttt{random} in each thread and causes 40X slowdown in user's experiments\footnote{http://bugs.mysql.com/bug.php?id=38941}.
\begin{comment}
\begin{enumerate}
  \item \underline{\emph{Configuration problem}}, a problem caused by external factors, rather than the application itself. These factors include hardware issues, such as insufficient memory or processing power; network issues, such as high latency, low throughput, and connection problems; and software problems, such as poorly tuned databases. For instance, in the case where the number of threads is greater than that of cores, the same code segment, as shown in Figure~\ref{fig:null_lock}, would generate different number of ISOs with the varying number of cores.
  \item \underline{\emph{Others}}. The broader terms: in fact, the occurrence of ISO attributes to the shared memory model. Based on it, a variety of high-level programming models (e.g., C/C++) are more or less defective. In recent years, this promising topic gets prevalent, such as transaction memory which runs programs in the form of the transaction without using synchronization primitives.
\end{enumerate}
\end{comment}
%In this paper, we mainly focuses on the identification and improvement of coding problems for developers.

\subsection{Implications}
%\indent\textbf{Why do we focus on ISO-performance problems?}
%Bugs with ISO-problems usually have severe performance impact. The reason is that ISO bugs usually serialize a large number of parallelizable codes, which amplifies the performance penalty of program. For \texttt{null-lock} pattern and a part of \texttt{read-read} pattern, worse still, lock synchronization introduces another aspect of performance penalty (synchronization overhead). For instance, in our unit testing on microbenchmark, we find that the optimization of \texttt{null-lock}, \texttt{read-read}, \texttt{irrelevant write-being} patterns can be improves by 50\%, 19.6\% and 24\% respectively, the valid time for real task being about 6.4\%.

%\textbf{Do you know if you have maximized your application's performance for the ISO-free case?}
%Not all applications suffer from the ISO-problems, with the scientific computing applications serving as the example that they
%scarcely contain synchronization operations. Accordingly, it is of no necessity to explore ISO-problems for this type of applications. The premise of our study, therefore, is to find out the optimizable applications, leaving out the ones without optimization value. When the targets are locked, we will then search for ways to improve the performance of these applications to the optimum.

%\textbf{How can we detect ISO-performance problems?}

ISOs are a special manifestation of the thread interleaving, which is featured by the mutually exclusive lock synchronization. Due to the diversity and complexity of thread interleavings, it is hard to explore all potential cases.
%\footnote{The exploration of all thread interleavings in multi-threaded applications is a NP-hard problem.}.
To be aware of thread interleaving, some static techniques are proposed, such as recording-based methods and data flow-based graph. These proposals are able to perceive \emph{why} and \emph{how} a thread interleaving occurs using a complete analysis. However, they can not accurately point out \emph{whether} an ISO actually happens, and can not count \emph{how often} a certain ISO, which may lead to a great performance impact, will happen.

To tackle this problem, we leverage the dynamic approach to pinpoint the performance impact of ISO problem at runtime. Different categories of ISOs may be eliminated by different methods in the face of different issues (discussed in Section~\ref{sec:elmination}). E.g., null-lock usually introduces synchronization overhead. Worse still, a more fetal problem---serial execution penalty, occurs when it uses the same lock and is executed by more than two threads concurrently. Generally, this bug can be fixed by eliminating the redundant lock. read-read pattern results in the same serial execution penalty. However, the fixing strategy is different. In general, we can also eliminate the lock to fix it in some cases, but sometimes this practice introduces potential data races. Therefore a more detailed causality should be analyzed to fix read-read pattern. Irrelevant write-being pattern consists of two cases: 1) irrelevant read-write, 2) and irrelevant write-write. Considering the definition of a data race, this bug could be fixed using different locks for different shared variables. To facilitate the implementation of the approaches above, a record/replay framework is presented in next Section~\ref{sec:perfplay}.
\begin{figure}[tb] %Figure 1
\centering
\includegraphics[scale=0.6]{fig/overview.eps}
\caption{Overview of \textsc{PerfPlay}}
\label{fig:overview}
\end{figure} 
